Improved Algorithms for Distributed Entropy Monitoring

Modern data management systems often need to deal with massive, dynamic and inherently distributed data sources. We collect the data using a distributed network, and at the same time try to maintain a global view of the data at a central coordinator using a minimal amount of communication. Such applications have been captured by the distributed monitoring model which has attracted a lot of attention in recent years. In this paper we investigate the monitoring of the entropy functions, which are very useful in network monitoring applications such as detecting distributed denial-of-service attacks. Our results improve the previous best results by Arackaparambil et al. [2]. Our technical contribution also includes implementing the celebrated AMS sampling method (by Alon et al. [1]) in the distributed monitoring model, which could be of independent interest.

==> preliminary.tex <==
\section{Preliminaries}
\label{sec:preliminary}
In this section we present some utility algorithms in distributed monitoring that will be used later.
\vspace{2mm}

\noindent{\bf \CEN.}
A simple (folklore) algorithm for counting the frequency of a given element in distribution monitoring is the following: Each site $S_i$ maintains a local counter $ct_i$, initiated to be $1$. Every time $ct_i$ increases by a factor of $(1+\eps)$, $S_i$ sends a message (say, a bit) to the coordinator. It is easy to see that the coordinator can always maintain a $(1+\eps)$-approximation of $\sum_i ct_i$, which is the frequency of the element. The total communication cost can be bounded by $O(k \cdot \log_{1+\eps} m) = O(k/\eps \cdot \log m)$ bits. The space used at each site is $\tilde{O}(1)$ bits and the processing time per item is $O(1)$. We denote this algorithm by \CEN$(e, \eps)$, where $e$ is the element whose frequency we want to track.

%\begin{lemma}[folklore] 
%\label{lem:CES}
%Given an element $e$, \CEN$(e, \eps)$  maintains a $(1+\epsilon)$-approximation to $e$'s frequency at the coordinator, using $O(\frac{k}{\eps} \log m)$ bits of communication, $O(1)$ space per site and $O(1)$ processing time per item.
%\end{lemma}

\vspace{3mm}

\noindent{\bf \CE.}
Huang et al.\ \cite{HYZ12} proposed a randomized algorithm \CE\ with a better performance. 

%We summarize their main result in the following lemma. 

%We will further denote this algorithm as $\text{\CE}(e, \eps,\delta)$. 

\vspace{-2mm}

\begin{lemma}[\cite{HYZ12}]
  \label{lem:CE}
Given an element $e$, $\text{\CE}(e, \eps,\delta)$ maintains a $(1+\epsilon, \delta)$-approximation to $e$'s frequency at the coordinator, using $\tilde{O}( k + \frac{\sqrt{k}}{\epsilon})$ bits of communication, $\tilde{O}(1)$ bits space per site and amortized $O(1)$ processing time per item.
%where $m$ is the length of union of $k$ streams.
\end{lemma}
For $S \subseteq [n]$, \CE$(S, \eps) = \sum_{e \in S} \text{\CE} (e, \eps)$, \CEN$(S, \eps) = \sum_{e \in S} \text{\CEN} (e, \eps)$.

\vspace{4mm}

\noindent{\bf\CA.}
Yi and Zhang \cite{YZ09} gave a deterministic algorithm, denoted by \CA$(\eps)$, that can be used to tracks the empirical probabilities of all universe elements up to an additive error $\eps$ in distributed monitoring. 

%We summarize their main result below.
\vspace{-2mm}

\begin{lemma}[\cite{YZ09}]
  \label{lem:CA}
For any $0 < \eps \leq 1$, \CA$(\eps)$ uses  $\tilde{O}(\frac{k}{\eps})$ bits of communication,
such that for any element $i \in [n]$, it maintains at the coordinator an estimation $\hat{p_i}$ such that
$\abs{\hat{p_i} - p_i} < \eps$. Each site uses $\tilde{O}(1/\eps)$ bits space and amortized $O(1)$ time per item.
\end{lemma}
\vspace{2mm}

\noindent{\bf\CM.}
We will also need  the  CountMin Sketch introduced by Cormode and Muthukrishnan \cite{cormode05}  in the streaming model. 
%We summarize its property below.
\vspace{-1mm}
\begin{lemma}[\cite{cormode05}]
  \label{lem:CM}
  The \CM$(\eps,\delta)$  sketch uses $\tilde{O}(\frac{1}{\eps})$ bits of space in the streaming model, such that for any given element $i \in [n]$, it gives an estimation $\hat{m}_i$ of $i$'s frequency $m_i$ such that
%  \begin{equation*}
%    \label{eq:cm}
    $\Pr[m_i \leq \hat{m}_i \leq m_i + \eps m_{-i}] \ge 1 - \delta$.
%  \end{equation*}
The processing time for each item is $O(1)$.
\end{lemma}


\vspace{2mm}

%\chensays{The following lemma only used inside Sampling in Sliding Window, which is treated as a black box. Do we need to keep this lemma?}

% \noindent{\bf\TRSH.}
% In the sequence-based sliding window, for each item received by the coordinator, it is possible to catch the event that the item expires in a timely manner. 

% \begin{lemma}[\cite{CMY11}, \cite{CMYZ12}]
% There is a deterministic algorithm \TRSH\ for the sequence-based sliding window that can be used to determine whether an item maintained at the coordinator expires or not, using $O(k \log w)$ bits of communication, each site will use $O(1)$ space and $O(1)$ time per item.
% \end{lemma}


%\vspace{2mm}

\noindent{\bf\em AMS-Sampling.} 
\label{pre:ams}
Recall the AMS-sampling framework sketched in the introduction. Define $\text{\Est}(f, R, \kappa) = \frac{1}{\kappa} \sum_{i \in [\kappa]} X_i$, where $\{X_1, \ldots, X_\kappa\}$ are i.i.d.\ sampled from the distribution of $X = f(R) - f(R-1)$. 
\begin{lemma}[\cite{CCM10}]
  \label{lem:c}
  Let $a\geq 0, b > 0$ such that $-a \leq X \leq b$, and
  \begin{equation}
    \label{eq:inq:c}
    \kappa \geq \frac{3(1 + a/\E[X])^2\eps^{-2}\ln(2\delta^{-1})(a + b)}{(a + \E[X])}.
  \end{equation}
If $\E[X] > 0$, then $\text{\Est}(f, R, \kappa) = \frac{1}{\kappa} \sum_{i \in [\kappa]} X_i$ gives a $(1 + \eps, \delta)$-approximation to $\E[X] = \bar{f}(A)$.

%If we further have $X = f(R) - f(R-1)$, then the estimator $\text{\Est}(f, R, \kappa)$ gives a $(1 + \eps, \delta)$-approximation to $\E[X] = \bar{f}(A) = \frac{1}{m}\sum_{i=1}^n f(m_i)$.
\end{lemma}



